SCOMatch: Alleviating Overtrusting in Open-set Semi-supervised Learning

Open-set semi-supervised learning (OSSL) leverages practical open-set unlabeled data, comprising both in-distribution (ID) samples from seen classes and out-of-distribution (OOD) samples from unseen classes, for semi-supervised learning (SSL). Prior OSSL methods initially learned the decision boundary between ID and OOD with labeled ID data, subsequently employing self-training to refine this boundary. These methods, however, suffer from the tendency to overtrust the labeled ID data: the scarcity of labeled data caused the distribution bias between the labeled samples and the entire ID data, which misleads the decision boundary to overfit. The subsequent self-training process, based on the overfitted result, fails to rectify this problem. In this paper, we address the overtrusting issue by treating OOD samples as an additional class, forming a new SSL process. Specifically, we propose SCOMatch, a novel OSSL method that 1) selects reliable OOD samples as new labeled data with an OOD memory queue and a corresponding update strategy and 2) integrates the new SSL process into the original task through our Simultaneous Close-set and Open-set self-training. SCOMatch refines the decision boundary of ID and OOD classes across the entire dataset, thereby leading to improved results. Extensive experimental results show that SCOMatch significantly outperforms the state-of-the-art methods on various benchmarks. The effectiveness is further verified through ablation studies and visualization.

==> tabs/tab5.tex <==
\begin{table*}[t]
\begin{center}
\caption{Ablation studies of components in SCOMatch.}
\label{tab:tab5}
\begin{tabular}{c|ccc|ccc}
\toprule
 \multirow{2}{*}{OOD score} & \multicolumn{3}{c|}{CIFAR-10} & \multicolumn{3}{c}{CIFAR-100}\\
\cline{2-7}
  & ACC$_{close}$ & ACC$_{open}$ & AUC & ACC$_{close}$ &  ACC$_{open}$ & AUC \\
\hline
 MSP ($\mathcal{C}^K$)  & 81.1 & 48.7 & 54.4 \\
 %Energy ($\mathcal{C}^K$) &      &      &    \\
 MSP ($\mathcal{C}$)    &      &      &      \\
 %Energy ($\mathcal{C}$)    &      &      &      \\  
\midrule
OpenMSP                & 76.5 & 70.5 & 91.9 \\

\bottomrule
\end{tabular}
\end{center}
\end{table*}

==> tabs/tab_sup_1.tex <==
\begin{table*}[t]
\centering
\begin{center}
\caption{Hyper-parameters used in SCOMatch.}
\label{tab:tab_sup_1}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c}
\toprule
& Hyper-parameter & Description    & MNIST    & CIFAR-10/100 & TinyImageNet & IN30 \\
\midrule
\multirow{7}{*}{\rotatebox{90}{SSL~(FixMatch)}} & $\tau$ & SSL confidence threshold & \multicolumn{4}{c}{0.95} \\
 & $\lambda$ & Unsupervised loss weight & \multicolumn{4}{c}{1} \\
 & $\beta$ & Momentum & \multicolumn{4}{c}{0.9} \\
 & $\alpha$ & EMA weight & \multicolumn{4}{c}{0.999} \\
 & Weight decay & Weight decay & \multicolumn{4}{c}{0.0005} \\
\cmidrule{4-7}
 & $lr$ & Learning rate & 0.001 & \multicolumn{3}{c}{0.03} \\
 & $B$ & Labeled data batch size & 50 & \multicolumn{3}{c}{64} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{Ours}} & $K_m$ & No. of enqueue samples per iter  & \multicolumn{4}{c}{1} \\
& $N_m$ & OOD memory queue length  & \multicolumn{4}{c}{8 $\times$ number of ID classes} \\
\cmidrule{4-7}
  & $\tau^{min}$ & Min value of $\tau^{ood}$ & 0.8 & \multicolumn{3}{c}{0.75}  \\

 & $\tau^{ood}$ & Confidence threshold for OOD class  & 0.8 & \multicolumn{3}{c}{CPL based threshold}  \\

 
 \bottomrule
\end{tabular}
}
\end{center}
\end{table*}
